Electron Acceleration and Radiation Generation from Relativistic Laser-Plasma Interactions at High Repetition-Rate

This dissertation explores the interaction between high-intensity lasers and plasmas to accelerate electrons and produce radiation via experimental and computational efforts. The laser pulses used in this dissertation have ultrashort duration (< 100 fs), near-infrared to mid-infrared wavelength (0.8 $\mu$m, 2 $\mu$m, or 3.9 $\mu$m), millijoules of energy, and high repetition rates (480 Hz or 20 Hz). The plasma sources applied are from solid-density targets (overdense) or gaseous targets (underdense). With the high-repetition-rate capability, statistical methods are employed to optimize certain aspect of the experiments and to interpret the physics.

==> abbr.tex <==

\acro{LWFA}{laser-wakefield acceleration}
\acro{LWFAs}{Laser-wakefield accelerators}
\acro{SM-LWFA}{Self-modulated laser-wakefield acceleration}
\acro{PWFA}{plasma-wakefield acceleration}
\acro{DLA}{direct laser acceleration}
\acro{CUOS}{Center for Ultrafast Optical Science}
% \acro{$\lambda^3$}{the $\lambda^3$ laser facility}
\acro{Lambda-cubed}{relativistic lambda cubed laser facility}
\acro{HHG}{High-order Harmonic Generation}
\acro{SHG}{Second Harmonic Generation}
\acro{SH}{Second Harmonic}
\acro{OAP}{off-axis parabolic mirror}
\acro{VLA}{Vacuum laser acceleration}
\acro{OPA}{Optical parametric amplifier}
\acro{CPA}{Chirped pulse amplification}
\acro{OPCPA}{optical parametric chirped pulse amplification}
\acro{QED}{quantum electrodynamics}
\acro{SFQED}{strong-field quantum electrodynamics}
\acro{XFELs}{X-ray free-electron lasers}
\acro{FELs}{free-electron lasers}
\acro{ROM}{relativistic oscillating mirror}
\acro{CWE}{coherent wake emission}
\acro{CCD}{charge-coupled device}
\acro{FWHM}{full-width half-maximum}
\acro{PIC}{particle-in-cell}
\acro{MPI}{multi-photon ionization}
\acro{REMPI}{resonance-enhanced multi-photon ionization}
\acro{ATI}{above-threshold Ionization}
\acro{ASE}{amplified spontaneous emission}
\acro{AOPDF}{acousto-optic programmable dispersive filter}
\acro{WLC}{white light generation}
\acro{am-241}{americium-241}
\acro{MIR}{mid-infrared}
\acro{IR}{infrared}
\acro{AOS}{adaptive optical system}
\acro{DM}{deformable mirror}
\acro{GA}{genetic algorithm}
\acro{FOM}{figure of merit}
\acro{RF}{Random Forest}
\acro{DNN}{Deep Neural Network}
\acro{DJINN}{Deep Jointly-Informed Neural Network}
\acro{GP}{Gaussian Process}
\acrodef{RL}[RL]{reinforcement learning}
\acrodef{ML}[ML]{machine learning}
\acrodef{AWAKE}[AWAKE]{Advanced Wakefield}
\acro{ICF}{inertial confinement fusion}
\acro{LIBS}{laser-induced breakdown spectroscopy}
\acro{LINACs}{linear accelerators}
\acro{LCLS}{Linac coherent light source}
\acro{MCNPX}{Monte Carlo N-Particle eXtended}
\acro{COTR}{coherent optical transition radiation}
\acro{CEP}{carrier-envelope-phase}
\acro{CNN}{convolutional neural network}
\acro{PMT}{photomultiplier tube}
\acro{QOCT}{quantum optimal control theory}


==> listOfPublications.tex <==
% LIST OF PUBLICATIONS

This dissertation contains the following published articles and conference presentations. Manuscripts which are currently under review are indicated. Additional works that do not contribute directly to this dissertation buy cover related material are also listed.

% \citeMyPaper{lin2020towards}
\section*{Journal Publications With Peer Review Process}
\begin{enumerate}
  \item \textbf{Lin, J.}, Easter, J. H., Krushelnick, K., Mathis, M., Dong, J., Thomas, A. G. R., and Nees, J. (2018): Focus optimization at relativistic intensity with high numerical aperture and adaptive optics. Optics Communications, 421, 79-82. 
  \item \textbf{Lin, J.}, Ma, Y., Schwartz, R., Woodbury, D., Nees, J. A., Mathis, M., Thomas, A. G. R., Krushelnick, K., and Milchberg, H. (2019): Adaptive control of laser-wakefield accelerators driven by mid-IR laser pulses. Optics express, 27(8), 10912-10923.
  \item Beier, N., Nguyen, T., \textbf{Lin, J.}, Nees, J., Krushelnick, K., and Dollar, F. (2019): Relativistic short- pulse high harmonic generation at 1.3 and 2.1 $\mu$m wavelengths. New Journal of Physics, 21(4), 043052.
  \item  \textbf{Lin, J.}, Batson, T., Nees, J., Thomas, A. G. R., and Krushelnick, K. (2020): Towards isolated attosecond electron bunches using ultrashort-pulse laser-solid interactions. Scientific reports, 10(1), 1-11.
  \item  (\textit{Under Review}) \textbf{Lin, J.}, Qian, Q., Murphy, J., Hsu, A., Ma, Y., Hero, A., Thomas, A. G. R., and Krushelnick, K. (2020): Beyond optimization--supervised learning applications in relativistic laser-plasma experiments. arXiv preprint arXiv:2011.05866.
\end{enumerate}

% \section*{Submitted publications with peer review process}


% \section*{Publications Without Peer Review Process}


\section*{Conference Presentations}
\begin{enumerate}
  \item \textbf{Lin, J.}, Nees, J., Krushelnick, K., Dollar, F, and Nguyen, T., “High order harmonic generation with femtosecond mid-infrared laser”, America Physics Society Division of Plasma Physics (Oct 2017). [Poster]
  \item \textbf{Lin, J.}, Nguyen, T., Beier, N., J., Nees, J., Dollar, F, and Krushelnick, K., “Surface high order harmonic generation using ultrashort 2$\mu m$ laser pulses”, First LaserNetUs User Meeting (Aug 2018). [Poster]
  \item \textbf{Lin, J.}, Xiao, X., J., Nees, , Underwood, C., Yang, H., Thomas, A. G. R., Jovanovic, I, J., Krushelnick, K., “Relativistic laser-solid interaction: from near-infrared to mid-infrared”, America Physics Society Division of Plasma Physics (Oct 2018). [Poster]
  \item \textbf{Lin, J.}, Batson, T., Nees, J., Thomas, A. G. R., and Krushelnick, K., “Scaling relativistic laser-solid interaction using 30fs laser pulses”, America Physics Society Division of Plasma Physics (Nov 2019). [Poster]
  \item \textbf{Lin, J.}, and Krushelnick, K., “Attosecond electron bunch, mid-infrared LWFA and machine learning”, Shanghai Institute of Optics and Fine Mechanics (Jan 2020). [Invited talk]
  \item \textbf{Lin, J.}, Qian, Q., Murphy, J., Hsu, A., Hero, A., Thomas, A. G. R., and Krushelnick, K., “Towards predicting electron beam charge upon phase control in laser wakefield accelerators using supervised learning techniques”, America Physics Society Division of Plasma Physics (Nov 2020). [Talk]
  \item \textbf{Lin, J.}, Qian, Q., Murphy, J., Hsu, A., Ma, Y., Hero, A., Thomas, A. G. R., and Krushelnick, K., “Feature analysis for LWFA using supervised learning techniques”, Advanced Accelerator Concepts Seminar Series (Dec 2020) [Invited talk]
\end{enumerate}

\section*{Additional Work}
\begin{enumerate}
  \item Burger, M., Skrodzki, P. J., \textbf{Lin, J.}, Nees, J., Krushelnick, K., and Jovanovic, I. (2018): Intense laser filament-solid interactions from near-ultraviolet to mid-infrared. Optics express, 26(13), 16456- 16465.
  \item Finney, L. A., \textbf{Lin, J.}, Skrodzki, P. J., Burger, M., Nees, J., Krushelnick, K., and Jovanovic, I. (2021): Filament-induced breakdown spectroscopy signal enhancement using optical wavefront control. Optics Communications, 126902
  \item (Accepted) Englesbe, A., \textbf{Lin, J.}, Nees, J., Lucero, A., Krushelnick, K., and Schmitt-Sody, A.(2021): Optimization of Microwave Emission from Laser Filamentation with a Machine Learning Algorithm. Applied Optics
\end{enumerate}

